Neural Academic Paper Generation

In this work, we tackle the problem of structured text generation, specifically academic paper generation in $\LaTeX{}$, inspired by the surprisingly good results of basic character-level language models. Our motivation is using more recent and advanced methods of language modeling on a more complex dataset of $\LaTeX{}$ source files to generate realistic academic papers. Our first contribution is preparing a dataset with $\LaTeX{}$ source files on recent open-source computer vision papers. Our second contribution is experimenting with recent methods of language modeling and text generation such as Transformer and Transformer-XL to generate consistent $\LaTeX{}$ code. We report cross-entropy and bits-per-character (BPC) results of the trained models, and we also discuss interesting points on some examples of the generated $\LaTeX{}$ code.

==> lstm-output-2.tex <==
We further analyze the effect of obtaining the proposed approach of our method and fine-tuning the spatial relationship between the surface instead of the annotation error \textbf{(as provided by the original image)} which are shown in Fig.~\textbf{\ref\{fig:runtime\}}. The second step is trained on the training set in a standard environment with a single sample image of the same size with a single color \textbf{(blue)} are present in the image. We then evaluated the performance of the pre-trained CNN features to obtain better performance than the state-of-the-art face recognition model in the appendix.

==> xl-output-2.tex <==
We verify the effectiveness of our proposed method on both the 50k \emph{and} the 2012 dataset available, all reported a reference performance of $66.1\%$ on the validation set. We also drop our initial performance (denoted as RPN $\stackanchor{+}{}$) and add RRCN \textbf{$\stackanchor{+}{}$} to get an average performance according to the three evaluation metrics. Results are shown in Table~\ref{tab:accuracy}. The three evaluation metrics are measured by computing the average, and showing the difference of RRCN with respect to the obtained initial performance (denoted as \textit{initial performance}).
